Analyzing (In)Abilities of SAEs via Formal Languages

Autoencoders have been used for finding interpretable and disentangled features underlying neural network representations in both image and text domains. While the efficacy and pitfalls of such methods are well-studied in vision, there is a lack of corresponding results, both qualitative and quantitative, for the text domain. We aim to address this gap by training sparse autoencoders (SAEs) on a synthetic testbed of formal languages. Specifically, we train SAEs on the hidden representations of models trained on formal languages (Dyck-2, Expr, and English PCFG) under a wide variety of hyperparameter settings, finding interpretable latents often emerge in the features learned by our SAEs. However, similar to vision, we find performance turns out to be highly sensitive to inductive biases of the training pipeline. Moreover, we show latents correlating to certain features of the input do not always induce a causal impact on model's computation. We thus argue that causality has to become a central target in SAE training: learning of causal features should be incentivized from the ground-up. Motivated by this, we propose and perform preliminary investigations for an approach that promotes learning of causally relevant features in our formal language setting.

==> name.tex <==
\begin{figure*}
\vspace{-15mm}
\captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_pos_frac_15.pdf}
    \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_pos_frac_8.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_pos_frac_4.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_pos_frac_2.pdf}
        \caption{}
    \end{subfigure}
    \vspace{5mm}
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_gram_15.pdf}
    \caption{(a) 15/15}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_gram_8.pdf}
        \caption{(b) 8/15}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_gram_4.pdf}
        \caption{(c) 4/15}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adj_gram_2.pdf}
        \caption{(d) 2/15}
    \end{subfigure}

    \vspace{5mm}
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_pos_frac_5.pdf}
    \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_pos_frac_4.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_pos_frac_3.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_pos_frac_2.pdf}
        \caption{}
    \end{subfigure}
    \vspace{5mm}
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_gram_5.pdf}
    \caption{(e) 5/5}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_gram_4.pdf}
        \caption{(f) 4/5}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_gram_3.pdf}
        \caption{(g) 3/5}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_verb_gram_2.pdf}
        \caption{(h) 2/5}
    \end{subfigure}

    \vspace{5mm}
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_pos_frac_13.pdf}
    \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_pos_frac_7.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_pos_frac_4.pdf}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_pos_frac_2.pdf}
        \caption{}
    \end{subfigure}
    \vspace{5mm}
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_gram_13.pdf}
    \caption{(i) 13/13}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_gram_7.pdf}
        \caption{(j) 7/13}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_gram_4.pdf}
        \caption{(k) 4/13}
    \end{subfigure}
    ~
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=0.9\linewidth]{figures/causality/caus_adv_gram_2.pdf}
        \caption{(l) 2/13}
    \end{subfigure}
    \caption{\textbf{Causal effects of \textbf{adjectives} ((a)-(d)), \textbf{verbs} ((e)-(h)), and \textbf{adverbs} ((i)-(l)).} The caption of each image describes the number of latents being intervened on. At each clamp value (x-axis), we plot the distribution of \textcolor{blue}{nouns}, \textcolor{orange}{pronouns}, \textcolor{green}{adjectives}, \textcolor{red}{verbs}, \textcolor{violet}{adverbs}, and \textcolor{brown}{conjunctions} (top) and the percentage of grammatical generations (bottom).}
\label{fig:causal_effects}
\end{figure*}
